Learning stability guarantees for constrained switching linear systems from noisy observations

We present a data-driven framework based on Lyapunov theory to provide stability guarantees for a family of hybrid systems. In particular, we are interested in the asymptotic stability of switching linear systems whose switching sequence is constrained by labeled graphs, namely constrained switching linear systems. In order to do so, we provide chance-constrained bounds on stability guarantees, that can be obtained from a finite number of noisy observations. We first present a method providing stability guarantees from sampled trajectories in the hybrid state-space of the system. We then study the harder situation where one only observes the continuous part of the hybrid states. We show that in this case, one may still obtain formal chance-constrained stability guarantees. For this latter result we provide a new upper bound of general interest, also for model-based stability analysis

==> content/A_proofs.tex <==
\section{Proofs of Section~\ref{hybridStates}}
\subsection{Proof of Proposition~\ref{PAC1}}
\begin{proof}
	\todoshort
\end{proof}

\subsection{Proof of Proposition~\ref{nonoise}}
\begin{proof}
	First we prove that if 
	\begin{equation}
		\| A_{\mathcal{L}(e)}x\|_{P_{t(e)}} > \left(\gamma + \sqrt{\frac{\lambda^{\max}\left(P_{t(e)}\right)}{\lambda^{\min}\left(P_{s(e)}\right)}}\|w\| \right) \| x \|_{P_{s(e)}}
	\end{equation}
	for any $(x, e, w) \in \omega$, $\gamma \in   \mathbb{R}_{>0}$ and $\{P_u\}_{u \in \mathcal{U}}$, then $\| A_{\mathcal{L}(e)}x + w\|_{P_{t(e)}} > \gamma \| x \|_{P_{s(e)}}$. For the sake of readability, let $\kappa = \sqrt{\lambda^{\max}\left(P_{t(e)}\right)/\lambda^{\min}\left(P_{s(e)}\right)}$ and $y = A_{\mathcal{L}(e)}x$. From subadditivity of the norm, it holds that 
	\begin{align}
		(\gamma + \kappa \|w\|)\|x\|_{P_{s(e)}} &< \|y + w - w\|_{P_{t(e)}} \\
		\implies (\gamma + \kappa \|w\|)\|x\|_{P_{s(e)}} &< \|y + w\|_{P_{t(e)}} + \|w\|_{P_{t(e)}}.
	\end{align}
	Now, it is a well known fact that, for any vector $x \in \mathbb{R}^n$ and matrix $P \in \mathcal{S}^n$, $\sqrt{\lambda^{\min}(P)}\|w\| \leq \|w\|_P \leq \sqrt{\lambda^{\max}(P)}\|w\|$. Therefore, 
	\begin{equation}
		\gamma \|x\|_{P_{s(e)}} + \kappa \|w\| \sqrt{\lambda^{\min}\left(P_{s(e)}\right)} < \|y + w\|_{P_{t(e)}} + \sqrt{\lambda^{\max}\left( P_{t(e)} \right)}\|w\|.
	\end{equation}
	From the definition of $\kappa$, the first step is proven. It remains to notice that, by definition, $\kappa \leq \overline{\kappa}(\omega)$ for all $(x, e, w) \in \omega$, and $\|w\| \leq W$ since $w \in B[0, W]$, and we get the desired result.
\end{proof}

\subsection{Proof of Corollary~\ref{PAC2}}
\begin{proof}
	It is equivalent to prove that, if
	\begin{equation}
		\tilde{\lambda}_l(\tilde{V}(\tilde{\omega}_N)) \leq \varepsilon(\beta, N).
	\end{equation}
	holds with some probability $\beta$, then
	\begin{equation}
		\lambda_l(V(\tilde{\omega}_N)) \leq \varepsilon(\beta, N).
	\end{equation}
	holds with the same probability. First, following Proposition~\ref{nonoise}, 
	\begin{equation}
		V(\tilde{\omega}_N) \times B[0, W] \subseteq \tilde{V}(\tilde{\omega}_N), 
	\end{equation}
	which implies that
	\begin{equation}
		\tilde{\lambda}^{(l)}\left(V(\tilde{\omega}_N) \times B[0, W]\right) \leq \tilde{\lambda}^{(l)}(\tilde{V}(\tilde{\omega}_N)).
	\end{equation}
	Since $\tilde{\lambda}^{(l)}\left(V(\tilde{\omega}_N) \times B[0, W]\right) = \lambda^{(l)}(V(\tilde{\omega}_N))$, then 
	\begin{equation}
		\lambda^{(l)}(V(\tilde{\omega}_N)) \leq \tilde{\lambda}^{(l)}(\tilde{V}(\tilde{\omega}_N)).
	\end{equation}
	So if $\tilde{\lambda}^{(l)}(\tilde{V}(\tilde{\omega}_N)) \leq \varepsilon$ for some $\varepsilon \in (0, 1)$ with some probability $\beta \in (0, 1)$, then so is $\lambda^{(l)}(V(\tilde{\omega}_N))$, and the proof is completed.
\end{proof}

\section{Proofs of Section~\ref{continuousStates}}

\subsection{Proof of Proposition~\ref{lifting}}
\begin{proof}
	First we prove inequality~\eqref{finiteIneq}. Since for all $t > 0$ and $l > 0$, $\mathcal{A}^{(lt)} \subseteq \left(\mathcal{A}^{(l)}\right)^t$, the definition of the JSR \todo{Define the JSR as well} yields 
\begin{equation}
\begin{aligned}
	\rho(\mathcal{A}^{(l)}) 	&= \lim_{t \to \infty} \max \left\{ \| A \|^{1/t}: \, A \in \left(\mathcal{A}^{(l)}\right)^t \right\} \\
					&\geq \lim_{t \to \infty} \max \left\{ \| A \|^{1/t}: \, A \in \mathcal{A}^{(lt)} \right\}.			
\end{aligned}					
\end{equation}
Letting $k := lt$ and using the definition of the CJSR (see Definition~\ref{CJSRdef}), the inequality becomes
\begin{equation}
\begin{aligned}
	\rho(\mathcal{A}^{(l)}) 	&\geq \lim_{t \to \infty} \max \left\{ \| A \|^{l/k}: \, A \in \mathcal{A}^{(k)} \right\} \\
					&= \left( \lim_{k \to \infty} \max \left\{ \| A \|^{1/k}: \, A \in \mathcal{A}^{(k)} \right\} \right)^l \\
					&= \rho(\mathcal{G}, \mathcal{A})^l, 
\end{aligned}
\end{equation}
which is the desired result. Now we prove asymptotic equality~\eqref{asymEq}. First, given another definition of the JSR \todo{Give the other definition of the JSR} for any $l > 0$,
\begin{equation}
\begin{aligned}
	\rho(\mathcal{A}^{(l)}) &\leq \max \left\{ \| A \|: \, A \in \mathcal{A}^{(l)} \right\} \\
	\iff \rho(\mathcal{A}^{(l)})^{1/l} &\leq \max \left\{ \| A \|^{1/l}: \, A \in \mathcal{A}^{(l)} \right\}.
\end{aligned}
\end{equation}
Taking the limit in both sides, it gives $\lim_{l \to \infty} \rho(\mathcal{A}^{(l)})^{1/l} \leq \rho(\mathcal{G}, \mathcal{A})$. Since $\rho(\mathcal{A}^{(l)})^{1/l} \geq \rho(\mathcal{G}, \mathcal{A})$ for any $l > 0$, it gives the desired result.
\end{proof}

